Adversarial Contrastive Learning via Asymmetric InfoNCE

Contrastive learning (CL) has recently been applied to adversarial learning tasks. Such practice considers adversarial samples as additional positive views of an instance, and by maximizing their agreements with each other, yields better adversarial robustness. However, this mechanism can be potentially flawed, since adversarial perturbations may cause instance-level identity confusion, which can impede CL performance by pulling together different instances with separate identities. To address this issue, we propose to treat adversarial samples unequally when contrasted, with an asymmetric InfoNCE objective ($A-InfoNCE$) that allows discriminating considerations of adversarial samples. Specifically, adversaries are viewed as inferior positives that induce weaker learning signals, or as hard negatives exhibiting higher contrast to other negative samples. In the asymmetric fashion, the adverse impacts of conflicting objectives between CL and adversarial learning can be effectively mitigated. Experiments show that our approach consistently outperforms existing Adversarial CL methods across different finetuning schemes without additional computational cost. The proposed A-InfoNCE is also a generic form that can be readily extended to other CL methods. Code is available at https://github.com/yqy2001/A-InfoNCE.

==> sections/intro.tex <==
\section{Introduction}

%%% 第一段，介绍鲁棒性是什么，缺乏鲁棒性有什么危害，对抗防御的意义：尽管神经网络非常非常牛，但遭受攻击时会很脆弱。目前主要防御手段是什么什么，局限是什么：都依赖于有标签数据、非常慢
% 第一句 尽管DNN展现出了非常好的性能，但面对Adversarial Examples时很脆弱；
% 第二句 什么是Adversarial Examples, 怎么构建出来的
% 第三句 DNN面对AE的脆弱性会带来很严重的危害
% 第四句 防御AE/adversarial attack的有效方法
% 第五句 这个有效方法存在一定的局限，为本文做的事情做铺垫

Though Deep Neural Networks (DNNs) have exhibited highly expressive performance and even surpass humans on many tasks, they are rigorously challenged by their vulnerability to \textit{adversarial examples} \cite{szegedy2014intriguing,goodfellow2014explaining}, which are artificially crafted to mislead the state-of-the-art models into incorrect predictions.
DNN's weakness in the face of adversarial examples poses severe threats to their applications in security-critical systems, e.g. autonomous driving, surveillance and face recognition~\cite{akhtar2018threat,kurakin2018adversarial,cao2019adversarial,vakhshiteh2020threat}.
One of the most powerful defense strategies against adversarial attacks is adversarial training (AT)~\cite{kannan2018adversarial,shafahi2019adversarial,zhang2019you,wong2020fast,zhang2019theoretically,zhu2019freelb}, built upon a min-max optimization problem where the inner one constructs adversaries by maximizing the loss and the outer one fits the network's parameters to them by minimizing the expected loss~\cite{madry2018towards}. AT is effective yet highly depends on labeled data~\cite{chen2020adversarial,kim2020adversarial}.

%%% 第二段，讲使用无标签数据的重要性。robustness是模型现实落地必须考虑的问题，而现实场景中，很容易获得大量的无标签数据。最近有工作开始将版监督手段融入到对抗学习中，意图从无标签数据中习得鲁棒的模型点。然而完全从无标签数据中习得鲁棒的模型，仍然是一片未被探索的蓝海

How to leverage unlabeled data to perform AT is an important and worth-exploring problem~\cite{gowal2020self,chen2020adversarial}.
In real-world practice, we can easily acquire huge amounts of domain-related unlabeled data, while it is often highly expensive to get them labeled.
% How to leverage unlabeled data to train robust models is an important and economically beneficial problem.
Moreover, to emphasize the value of unlabeled data, some recent works claim that robustness should not inherently require labels because we essentially ask predictors to be stable around naturally occurring inputs~\cite{carmon2019unlabeled}, and they resort to semi-supervised learning to boost model's robustness \cite{alayrac2019labels,carmon2019unlabeled}. 
Nevertheless, these methods still require labeled images to generate pseudo-supervision for consequent adversarial training, and can be in essence regarded as fully-supervised adversarial training. How to train robust models totally from unlabeled data remains an important but less explored question.
Most recently, some works attempted to combine contrastive and adversarial training to perform AT on unlabeled data. The main idea is to generate adversaries against the contrastive loss first, then maximize the similarity between clean views and their adversarial counterparts~\cite{kim2020adversarial,fan2021does,jiang2020robust}.
% extend the conventional contrastive part to adversarial scenario where contrast is performed between adversarial view and clean view. 
RoCL\cite{kim2020adversarial} first proposed the above unlabeled AT scheme against contrastive loss and AdvCL\cite{fan2021does} propose to minimize the learning task gap between unlabeled contrast and labeled fintuning by introducing pseudo-supervision in pretraining stage, achiving the state-of-the-art performance.

\begin{figure}[t]
\centering
\includegraphics[scale=0.41]{images/intro图4.png}
% \includegraphics[width=\textwidth]{images/intro图.png}
\caption{
The schematic illustration for the conflict brought by adversarial contrastive learning and our proposed new views on adversaries to reduce such conflicts.
% The schematic illustration for the intrinsic properties of adversarial contrastive learning. Datapoints with same color belong to the same class. Triangles represent the adversaries, circles represent the benign images. 1) cats' representations (yellow circles) have tendencies to go towards other classes, and vice versa, leading to all classes shrink together; 2) adversaries can serve as other data points' hard negative, which have both different labels and similar representations (wrapped in dashed circle).
}
\label{fig:intro}
% \includegraphics[width=5cm, height=4cm]{overleaf-logo}
\end{figure}

%%% 第三段，介绍CL，CL在表示学习领域取得巨大的成功，跟我们的工作联系最紧密的CL+Adv的工作，介绍一下这几个工作
% 第一句，介绍CL是representation learning那边取得巨大突破的技术
% 第二句，最近的unsupervised adversarial 工作开始将CL融合进来
% 举例

% Contrastive Learning (CL), which attracts the same image's augmented views and repulses those of different images, has made encouraging progress in self-supervised representation learning.


%%% 第四段，这几个CL+adv的工作有什么局限：直接继承了传统CL，但ACL和CL是不同的，直接用对称的相似度会导致Random walking，lead to both acc drop，介绍我们的idea，我们觉得应该是怎么样，propose了什么，怎样改善这个局限，并自圆其说
% 第一句，当前CL+Adv工作的局限：直接继承了CL的做法而根本没有考虑CL和ACL的不同
% 第二句，在CL中是什么样的
% 第三句，我们觉得在ACL中不应该是CL这样
% 第四句，详细阐释
Although existing \textit{Adversarial Contrastive Learning} works have achieved satisfactory robustness in unlabeled settings, we argue that current simple
% introduction of adversarial into contrastive learning 
extension from contrastive learning to adversarial
doesn't treat adversaries correctly and brings severe conflicts in pretraining objectives. The adversaries in ACL are generated against the contrastive loss, i.e., they are away from the anchor as far as possible and pushed close to other datapoints, contrary to the CL's objective. Conventional CL pushes away an anchor with other data points, when we introduce adversarial learning, the contrast between adversaries and their anchors attract the anchors towards other data points that the adversaries are close to, which is a totally opposite direction against CL's exertion from the geometry perspective, as shown in Figure \ref{fig:intro}(b), engendering absolutely conflicts in training objective. Moreover, we will show by a limit case that current introduction of adversaries actually sets a potential objective to shrink all images into one point. The problem is rooted in that current adversarial contrastive learning treats adversaries the same as other clean augmentations and asks the anchors to head towards them.
% treats adversaries as good views.
% Simply put, conventional CL pushes a image away from other data points, adversarial comes and asks the sample to go towards other points, severely challenge conventional CL.

So how to take adversaries correctly in adversarial contrastive learning? We present two new treatments for adversaries from the perspectives of both positives and negatives to alleviate this conflict. Firstly, as positives, we propose to view adversaries as \textit{inferior positives} that have asymmetric similarity with normal positives (clean augmentations) to directly reduce the conflict, as shown in Figure~\ref{fig:intro}(c). On the other hand, we propose to treat them as \textit{hard negatives} that should be upweighted when pushed away from other data points to further help relieve the conflict and make the model more robustness-aware, as shown in Figure~\ref{fig:intro}(d).

%should be pulled back but do not attract other clean views
When viewed as inferior positives, we propose that the similarity between clean views and adversarial views shouldn't be symmetric, i.e., we hope adversarial ones similar to clean ones and to be pulled back, but actually don't hope the model learns to represent clean images as adversaries which are intentionally perturbed. We put forward an adaptive gradient stopping strategy to model this asymmetry.
Moreover, we argue that adversarial views have excellent intrinsic properties to become hard negatives in which case they should be upweighted to make the model more robustness-aware. As proposed in \cite{robinson2020contrastive}, two principles to make a good negative sample for $x$ are: 1. "True negative" $x^-$ whose label differs from that of the anchor $x$; 2. The embedding currently believes to be similar to $x$.
Adversaries, as stated above, are often close to some other data points that could have different labels, satisfying our desire for hard negatives perfectly, what we need to do is to distinguish each data point from its surrounding other classes' adversarial views. Here we combine ideas of positive-unlabeled learning~\cite{du2014analysis,elkan2008learning} with adversarial and resort to the prevalent practice for reweighting negatives in contrastive learning \cite{robinson2020contrastive,chuang2020debiased}, to effectively sample true adversarial negatives and reweight each sample according to the current similarity.

%%% 第七段，summarize our contribution
To sum up, our contributions are as follows: 
\begin{itemize}
    \item We are the first to consider modeling the asymmetric property of \textit{Adversarial Contrastive Learning} and propose to perform asymmetric gradient stopping, which can boost both standard accuracy and robustness.
    \item We provide a new perspective for adversaies in contrastive learning, i.e., view them as hard negatives, which can also be extended to other adversarial scenarios.
    \item We present a generalized asymmetric InfoNCE loss: A-InfoNCE that unifies all current contrastive learning methods and can integrate our two proposed new views conveniently.
    \item Our methods are compatible with current adversarial contrastive learning methods, outperform the chosen baselines and achieve new state-of-the-art performance.
    %and outperform TRADES with only light-weight online finetuning.
\end{itemize}

% which is compatible with current adversarial CL methods, brings no extra computational overhead while significantly boosts both clean and robust accuracy.

% Although existing \textit{Contrastive Learning + Adversarial} works have achieved satisfactory robustness in unlabeled data settings, they are just directly inheriting CL's idea, together with its inherent deficiencies which is even enlarged, without in-depth study of the difference between \textit{CL} and \textit{Adversarial CL}. 
% Standard CL brings bad class discrimination because they perform instance discrimination task that pushes semantically similar pairs away\cite{chen2021large,chen2020self}. We claim that in Adversarial CL things get worse, we not only inheriting CL's deficiency to push away semantically similar pairs, but also attract representations from different classes.
% In standard Contrastive Learning, due to the random augmentation, two views of one image have same status and contribute to their similarity equally. When we maximize their similarity, we are actually pushing them heading towards each other together. 
% But in the adversarial scenario, we claim that, different from conventional CL, the \textbf{similarity between adversarial view and clean view shouldn't be symmetric}, which is totally ignored by previous works.
% Adversarial representations are to some extent "bad" representations that are produced intentionally by human to fool the model into outputting bad results. When we utilize CL to maximize similarity between a clean view and an adversarial view, our right action should be letting adversarial representations step towards the clean representations more rather than directly push them together. We want to let adversarial representations similar to clean ones, stable around clean representations, but actually don't hope the model learns to represent clean ones as adversaries which are intentionally perturbed.



% % 第五段，详细阐述危害
% Representation of a successful adversary can step across the classifier's hyperplane and land in another class's representation space. For example, as shown in Figure \ref{fig:intro}, a \textit{cat} image's representation lands in \textit{airplane}'s representation space after exerted adversarial perturbation and is misclassified as \textit{airplane}. If we don't consider the asymmetry and let the clean view and adversarial view forward towards each other, the optimization progress will push \textit{cat}'s representations heading towards \textit{airplane} and blur the classification boundary, bringing worse class discrimination and making an adversary easier to successfully attack the model. 
% More badly, take PGD as attack example, due to the random initialization, different adversarial perturbations may forward towards different directions, i.e. \textit{cat} is attacked into \textit{airplane} but next time \textit{truck}. If we always push two clean and adversarial representations together while don't have anchor points in representation space, the model's objective will \textbf{keep changing} (first let \textit{cat}s' representations forward towards \textit{airplane} and next time towards \textit{truck}), the learned representations will \textbf{keep random walking} and finally land in some unknown space. With such an \textbf{inconsistent} training objective, the difficulty of learning will increase and the model will feel largely confused. 
% % Moreover, the model's performance will drop obviously with larger epochs training due to the bad training objective.
% The example above demonstrate that \textit{cat}'s representations will forward towards \textit{airplane} then \textit{truck}, and vice versa, for \textit{airplane} and \textit{truck}, when they are served as clean anchors, they will go towards \textit{cat} too. In summary, without considering the asymmetry, we are actually \textbf{setting a potential objective for the model to push all classes together}. Adversarial CL has worse class discrimination because we not only push away semantically similar pairs, but also attract pairs with completely different semantics.
% % Inspired by the above analysis, we have an interesting finding that we can boost current Adversarial CL methods's both robust accuracy by over 1 points by simply reduce the training epoch by a half.

% %%% 第六段，proposal
% To this end, we propose that in \textit{Adversarial Contrastive Learning}, the contrast between clean views and adversarial views shouldn't be symmetric, what we want to do is pull all adversaries scattered in the representation space back and let the model learn to robustly represent images (represent the perturbed images near the clean ones). And we propose an adaptive gradient stopping strategy to model this asymmetry, which is compatible with current adversarial CL methods, brings no extra computational overhead while significantly boosts both clean and robust accuracy.

% Moreover, we provide a novel perspective for adversarial views in contrastive learning. We propose to treat adversarial views as \textit{hard negatives} to further enhance class discrimination. As proposed in \cite{robinson2020contrastive},
% two principles to make a good negative sample for $x$ are:
% 1. "True negative" $x_i^-$ whose label differs from that of the anchor $x$; 2. The most useful negative samples are ones that the embedding currently believes to be similar to the anchor.
% We argue that adversarial views have excellent intrinsic properties to become some other datapoints' hard negatives in which case they should be upweighted to make the model more robustness-aware, meanwhile bringing better class discrimination.
% For example, as shown in Figure \ref{fig:intro}, the yellow circle($x_1$) belongs to class \textit{cat}, its adversarial view $x_1^{adv}$(the yellow triangle), which attacks successfully, has definitely different representation from $x_1$ and is misclassified as \textit{airplane}. Then for some datapoints in \textit{airplane}, $x_1^{adv}$ is a natural hard negative that has both different label and similar representation. 
% \yqycomment{差转折词、这一段之后再配合图完善一下} What we need to do is to distinguish each datapoint from its surrounding adversarial views. Here we borrow ideas from positive-unlabeled learning and resort to the prevalent practice for reweighting negatives in Contrastive Learning \cite{robinson2020contrastive}, to effectively sample true negatives and reweight each sample according to the current similarity.


% %%% 第七段，summarize our contribution
% To sum up, our contributions are as follows: (TODO)
% \begin{itemize}
%     \item We are the first to consider modeling the asymmetric property of \textit{Adversarial Contrastive Learning} and propose to perform asymmetric gradient stopping, which can boost both standard accuracy and robustness.
%     \item We provide a new perspective for adversaies in contrastive learning, i.e., view them as hard negatives, which can also be extended to other adversarial scenarios.
%     \item Our methods are compatible with current adversarial contrastive learning methods and achieve the new state-of-the-art robustness accuracy.
%     %and outperform TRADES with only light-weight online finetuning.
% \end{itemize}


% % A more vivid scene: in representation space, the clean view wave to the adversarial one and said: "Hey, although we are derived from the same image, I want you similar to me, not I to you, because you are an artificial bad guy!"
